Fast Multi-frame Stereo Scene Flow with Motion Segmentation

We propose a new multi-frame method for efficiently computing scene flow (dense depth and optical flow) and camera ego-motion for a dynamic scene observed from a moving stereo camera rig. Our technique also segments out moving objects from the rigid scene. In our method, we first estimate the disparity map and the 6-DOF camera motion using stereo matching and visual odometry. We then identify regions inconsistent with the estimated camera motion and compute per-pixel optical flow only at these regions. This flow proposal is fused with the camera motion-based flow proposal using fusion moves to obtain the final optical flow and motion segmentation. This unified framework benefits all four tasks - stereo, optical flow, visual odometry and motion segmentation leading to overall higher accuracy and efficiency. Our method is currently ranked third on the KITTI 2015 scene flow benchmark. Furthermore, our CPU implementation runs in 2-3 seconds per frame which is 1-3 orders of magnitude faster than the top six methods. We also report a thorough evaluation on challenging Sintel sequences with fast camera and object motion, where our method consistently outperforms OSF [Menze and Geiger, 2015], which is currently ranked second on the KITTI benchmark.

==> tex_fig/fig_kitti_results.tex <==
\begin{figure*}
\centering
\footnotesize
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/10}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/finalseg0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/epidisp0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/10_derr}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/fullflo0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_02/10_ferr}\\
\vskip 0.5mm
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/10}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/finalseg0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/epidisp0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/10_derr}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/fullflo0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_06/10_ferr}\\
\vskip 0.5mm
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/10}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/finalseg0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/epidisp0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/10_derr}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/fullflo0}\hfill
\includegraphics[width=0.16\linewidth]{figures/KITTI_10/10_ferr}\\
\vskip 0.5mm
\makebox[0.16\linewidth]{(a) Input left image}\hfill
\makebox[0.16\linewidth]{(b) Motion segmentation $\myS$}\hfill
\makebox[0.16\linewidth]{(c) Disparity map $\myD$}\hfill
\makebox[0.16\linewidth]{(d) Disparity error map}\hfill
\makebox[0.16\linewidth]{(e) Flow map $\myF$}\hfill
\makebox[0.16\linewidth]{(f) Flow error map}\hfill
\vskip 0.5mm
\caption{Our results on KITTI training sequences \textit{000002}, \textit{000006} and \textit{000010}. Black pixels in error maps indicate missing ground truth.}
\label{fig:kitti_results}
\end{figure*}


==> tex_fig/fig_sintel_results.tex <==
\begin{figure*}[!t]
\scriptsize
\centering
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/ambush_5/image0}
\put(55,3){\textcolor{white}{\sf\textbf{ambush\_5}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/ambush_5/seg0}
\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/ambush_5/disp0}
\put(84,3){\textcolor{black}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/ambush_5/disp0}
\put(76,3){\textcolor{black}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/ambush_5/flow0}
\put(84,3){\textcolor{black}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/ambush_5/flow0}
\put(76,3){\textcolor{black}{\sf\textbf{Ours}}}
\end{overpic}
\vskip 0.5mm
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/ambush_5/seg0}
\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/ambush_5/seg0}
\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/ambush_5/disp0}
\put(71,3){\textcolor{black}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/ambush_5/disp0}
\put(77,3){\textcolor{black}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/ambush_5/flow0}
\put(71,3){\textcolor{black}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/ambush_5/flow0}
\put(77,3){\textcolor{black}{\sf\textbf{OSF}}}
\end{overpic}
%
\vskip 1.5mm
%
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/cave_4/image0}
\put(68,3){\textcolor{white}{\sf\textbf{cave\_4}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/cave_4/seg0}
\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/cave_4/disp0}
\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/cave_4/disp0}
\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/cave_4/flow0}
\put(84,3){\textcolor{black}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/cave_4/flow0}
\put(76,3){\textcolor{black}{\sf\textbf{Ours}}}
\end{overpic}
\vskip 0.5mm
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/cave_4/seg0}
\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/cave_4/seg0}
\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/cave_4/disp0}
\put(71,3){\textcolor{white}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/cave_4/disp0}
\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/cave_4/flow0}
\put(71,3){\textcolor{black}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/cave_4/flow0}
\put(77,3){\textcolor{black}{\sf\textbf{OSF}}}
\end{overpic}
%
\vskip 1.5mm
%
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/mountain_1/image0}
\put(48,3){\textcolor{white}{\sf\textbf{mountain\_1}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/mountain_1/seg0}
\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/mountain_1/disp0}
\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/mountain_1/disp0}
\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/mountain_1/flow0}
\put(84,3){\textcolor{black}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/mountain_1/flow0}
\put(76,3){\textcolor{black}{\sf\textbf{Ours}}}
\end{overpic}
\vskip 0.5mm
\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/mountain_1/seg0}
\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/mountain_1/seg0}
\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/mountain_1/disp0}
\put(71,3){\textcolor{white}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/mountain_1/disp0}
\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/mountain_1/flow0}
\put(71,3){\textcolor{black}{\sf\textbf{PRSM}}}
\end{overpic}\hfill
\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/mountain_1/flow0}
\put(77,3){\textcolor{black}{\sf\textbf{OSF}}}
\end{overpic}
%
%\vskip 1.5mm
%%
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/temple_2/image0}
%\put(60,3){\textcolor{white}{\sf\textbf{temple\_2}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/temple_2/seg0}
%\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/temple_2/disp0}
%\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/temple_2/disp0}
%\put(76,3){\textcolor{white}{\sf\textbf{Ours}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/temple_2/flow0}
%\put(84,3){\textcolor{black}{\sf\textbf{GT}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel_Ours/temple_2/flow0}
%\put(76,3){\textcolor{black}{\sf\textbf{Ours}}}
%\end{overpic}
%\vskip 0.5mm
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel___GT/temple_2/seg0}
%\put(84,3){\textcolor{white}{\sf\textbf{GT}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/temple_2/seg0}
%\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/temple_2/disp0}
%\put(71,3){\textcolor{white}{\sf\textbf{PRSM}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/temple_2/disp0}
%\put(77,3){\textcolor{white}{\sf\textbf{OSF}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel_PRSM/temple_2/flow0}
%\put(71,3){\textcolor{black}{\sf\textbf{PRSM}}}
%\end{overpic}\hfill
%\begin{overpic}[width=0.16\linewidth]{figures/Sintel__OSF/temple_2/flow0}
%\put(77,3){\textcolor{black}{\sf\textbf{OSF}}}
%\end{overpic}
\footnotesize
\makebox[0.32\textwidth]{Reference images / motion segmentation}\hfill
\makebox[0.32\textwidth]{Disparity maps}\hfill
\makebox[0.32\textwidth]{Flow maps}\hfill
\vskip 0.5mm
\caption{Comparisons on ambush\_5, cave\_4, mountain\_1 and temple\_ 2 from Sintel: [\textsc{Left}] Motion segmentation results -- ours, OSF and ground truth. [\textsc{Middle}] Disparity and [\textsc{Right}] Flow maps estimated by our method, PRSM and OSF and the ground truth versions.}
\label{fig:sintel_results}
\end{figure*}


==> tex_fig/tab_epipolar.tex <==
\begin{table}
\caption{Disparity improvements from binocular to epipolar stereo.
%We show average disparity error rates ($\%$) over 200 frames from KITTI training dataset.
}
\label{tab:epipolar}
\scriptsize
\vskip 0.5mm
\begin{tabular}{c|c|c|c|c|c|c}
 & \multicolumn{3}{|c|}{all pixels} & \multicolumn{3}{|c}{non-occluded pixels} \\ 
 & D1-bg & D1-fg & D1-all &  D1-bg & D1-fg & D1-all \\ \hline 
Binocular  ($\tilde{\myD}$) & 7.96 & 12.61 & 8.68 & 7.09 & 10.57 & 7.61 \\
Epipolar  (${\myD}$) & \textbf{5.82} & \textbf{10.34} & \textbf{6.51} & \textbf{5.57} & \textbf{8.84} & \textbf{6.06} \\ 
\end{tabular}
\end{table}


==> tex_fig/tab_kitti_scores.tex <==
\begin{table*}[t]
\caption{KITTI 2015 scene flow benchmark results~\cite{Menze2015}.
We show the error rates (\%) of the disparity on the reference frame (D1) and second frame (D2), the optical flow (Fl) and the scene flow (SF) in background (bg), foreground (fg) and all pixels.
Disparity or flow is considered correctly estimated if the end-point error is $<$ 3px or $<$ 5\%.
Scene flow is considered correct if D1, D2 and Fl are correct.
}
\label{tab:kitti_scores}
\scriptsize
\centering
\vskip 1mm
\begin{tabular}{c | c | c | c | c | c | c | c | c | c | c | c | c | c | c }
{\bf Rank} & {\bf Method} & {\bf D1-bg} & {\bf D1-fg} & {\bf D1-all} & {\bf D2-bg} & {\bf D2-fg} & {\bf D2-all} & {\bf Fl-bg} & {\bf Fl-fg} & {\bf Fl-all} & {\bf SF-bg} & {\bf SF-fg} & {\bf \textcolor{red}{SF-all}}  & {\bf Time} \\ \hline
1 & PRSM~\cite{Vogel2015} & \textbf{3.02} \ & \textbf{10.52} \ & \textbf{4.27} \ & \textbf{5.13} \ & \textbf{15.11} \ & \textbf{6.79} \ & \textbf{5.33} \ & \textbf{17.02} \ & \textbf{7.28} \ & \textbf{6.61} \ & \textbf{23.60} \ & \textbf{9.44} \  & 300 s \\
2 & OSF~\cite{Menze2015} & 4.54 \ & 12.03 \ & 5.79 \ & 5.45 \ & 19.41 \ & 7.77 \ & 5.62 \ & 22.17 \ & 8.37 \ & 7.01 \ & 28.76 \ & 10.63 \  & 50 min \\
3 & \textbf{FSF+MS} (ours) & 5.72 \ & 11.84 \ & 6.74 \ & 7.57 \ & 21.28 \ & 9.85 \ & 8.48 \ & 29.62 \ & 12.00 \ & 11.17 \ & 37.40 \ & 15.54 \  & 2.7 s \\
4 & CSF~\cite{Lv2016} & 4.57 \ & 13.04 \ & 5.98 \ & 7.92 \ & 20.76 \ & 10.06 \ & 10.40 \ & 30.33 \ & 13.71 \ & 12.21 \ & 36.97 \ & 16.33 \  & 80 s \\
5 & PR-Sceneflow~\cite{Vogel2013} & 4.74 \ & 13.74 \ & 6.24 \ & 11.14 \ & 20.47 \ & 12.69 \ & 11.73 \ & 27.73 \ & 14.39 \ & 13.49 \ & 33.72 \ & 16.85 \  & 150 s \\
8 & PCOF + ACTF~\cite{Derome2016} & 6.31 \ & 19.24 \ & 8.46 \ & 19.15 \ & 36.27 \ & 22.00 \ & 14.89 \ & 62.42 \ & 22.80 \ & 25.77 \ & 69.35 \ & 33.02 \  & 0.08 s \\
12 & GCSF~\cite{Cech2011} & 11.64 \ & 27.11 \ & 14.21 \ & 32.94 \ & 35.77 \ & 33.41 \ & 47.38 \ & 45.08 \ & 47.00 \ & 52.92 \ & 59.11 \ & 53.95 \  & 2.4 s \\
\end{tabular}\end{table*}


==> tex_fig/tab_sintel_scores.tex <==
\begin{table}
\centering
\caption{Evaluation on 21 video sequences from Sintel dataset~\cite{Butler2012}.
For each sequence, we show average error rates ($\%$) of disparity (D1), flow (Fl), scene flow (SF) and motion segmentation (MS) for all pixels over the frames. 
Colors of the cells of OSF~\cite{Menze2015} and PRSM~\cite{Vogel2015} scores illustrate
relative performances compared with our method; blue/red colors indicate our method is better/worse.
}
\label{tab:sintel_scores}
\vskip 1mm
\includegraphics[width=\linewidth]{figures/sintel_scores}
\end{table}
